SaDI: A Self-adaptive Decomposed Interpretable Framework for Electric Load Forecasting under Extreme Events

Accurate prediction of electric load is crucial in power grid planning and management. In this paper, we solve the electric load forecasting problem under extreme events such as scorching heats. One challenge for accurate forecasting is the lack of training samples under extreme conditions. Also load usually changes dramatically in these extreme conditions, which calls for interpretable model to make better decisions. In this paper, we propose a novel forecasting framework, named Self-adaptive Decomposed Interpretable framework~(SaDI), which ensembles long-term trend, short-term trend, and period modelings to capture temporal characteristics in different components. The external variable triggered loss is proposed for the imbalanced learning under extreme events. Furthermore, Generalized Additive Model (GAM) is employed in the framework for desirable interpretability. The experiments on both Central China electric load and public energy meters from buildings show that the proposed SaDI framework achieves average 22.14% improvement compared with the current state-of-the-art algorithms in forecasting under extreme events in terms of daily mean of normalized RMSE. Code, Public datasets, and Appendix are available at: https://doi.org/10.24433/CO.9696980.v1 .

==> sections/1.75_Problem_defination.tex <==





\section{Preliminary}
% @Linxiao
%\subsection{Task definition}
\paragraph{EPLF problem} We consider the scenario
referred to as ``day-ahead prediction'',
where the prediction on the day $T$ is required to be ready before the day $T-1$.
We note that day-ahead prediction is most common in reality, as power load prediction of the day $T$ is needed at the beginning of the day $T-1$ for scheduling of energy allocation. 
% the engineers need the prediction power load of the day $T$ on the day $T-1$ to make schedule of energy allocation. In day-ahead prediction, 
Given a collection of features, we aim to predict the energy load of the day $T$, i.e. $\{y_t\}_{t=0}^{m-1}$,
where $m$ denotes the number of data points collected in a day, usually equal to $96$ taken every $15$-mins. The features used to predict $y_t$
can be classified into two classes, i.e., historical features and external features. Specially, we denote $p$ historical features as $\{x_{t,i}\}_{i=0}^{p-1}$,
which encode the information of energy load before day $T-1$, and $q$ external features
as $\{x_{t,i}\}_{i=0}^{q-1}$, which include numerical weather prediction and information from the calendar, such as months, weekdays and special holidays.
Define $\boldsymbol{y}=[y_0,\dots,y_{m-1}]$,
$\boldsymbol{x}_t^h=[x_{t,0}^h,\dots,x_{t,p-1}^h]$,
$\boldsymbol{x}_t^e=[x_{t,0}^e,\dots,x_{t,q-1}^e]$,
and $\boldsymbol{x}_t=[(\boldsymbol{x}^h_t)^T,(\boldsymbol{x}^e_t)^T]^T$.
We aim to find a function $f(\cdot)$ such that the success rate of prediction
is maximized. A prediction is said to be successful if the normalized root mean square error is less than a predefined threshold $\eta$.
We denote the success rate with threshold $\eta$ as 
$\text{SR}@\eta$.
Then, given a set of
$\{(\boldsymbol{x}_t,y_t)\}$, we aim
to maximize:
\begin{align}\label{equ:success_rate}
    \text{SR}@\eta=\mathbb{E}\left[
    \mathcal{I}\left(\sqrt{\frac{1}{m}\sum_{t=0}^{m-1}\frac{(y_t-f(\boldsymbol{x}_t))^2}{y_t^2}}\leq\eta\right)
    \right]
\end{align}
where $\mathcal{I}(Q)$ is an indicator function that equals $1$ if $Q$ is true and $0$ otherwise. We note that directly optimizing $\text{SR}@\eta$ is difficult due to its non-differential property. To address this issue,
in the following section, we propose a decomposition-based model.
% to forecast the electricity load. 
Moreover, in order to enhance robustness against extreme events, we introduce a self-adaptive loss that can adaptively assign weights according to the fitting error of each time stamp. 

% To introduce our framework naturally, we introduce representative approaches first and show the necessities of our works.  ??

%omitted by yangyang
% \emph{Extreme Value Theory}: Extreme value theory or extreme value analysis (EVA) is a branch of statistics that deals with extreme deviations from the median of a probability distribution. Extreme Value Loss is applied widely, proposed by \cite{EVLoss/kdd19/} provides better predictions on future occurrences of extreme events. However, labels and features in time series cannot satisfy independent and identically distributed assumption of Extreme Value Theory, also this algorithm highly depending on hyper parameters. These two limitations lead to not very impressive performance in load forecasting under extremely events.




==> sections/1.85_motivation.tex <==
\section{Motivations}
\textcolor{red}{1. define the abstract problem we are dealing with in the tasks: overfitting, underfitting 2. vertical ensemble vs horizontal ensemble. horizontal is different function mapping to the same problem. vertical ensemble is decomposed the problem and map a different function to 
each sub-problem. Here our decomposed framework mainly dealing with the XX problem through 3. other motivations }

==> tables/tab_bench_evtloss.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table}[h]
\centering
\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Performance comparison under extreme event of SaDI and baselines on datasets of Hubei and Hunan. Best performance is highlighted in bold. A lower nRMSE indicates better performance.}
% \scalebox{0.85}{
%\resizebox{\linewidth}{!}{ 
\begin{tabular}{c|c|c|c|c}
\hline
% \toprule
nRMSE&\multicolumn{1}{c|}{SaDI}&\multicolumn{1}{c|}{LightGBM}&\multicolumn{1}{c|}{EVT}&\multicolumn{1}{c}{LDS}\\
\hline
\hline
% \midrule
% 1-nRMSE & 55days & 7days& 55days & 7days& 55days & 7days& 55days & 7days\\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$huazhong$}} 
% huazhong & \textbf{0.963} & \textbf{} & 0.952 & 0.  & 0.953 & & 0.953 & \\

% hubei-55days & \textbf{0.948}  & 0.934  & 0.937 & 0.937  \\

% hunan-55days & \textbf{0.954} & 0.956  & 0.946 & 0.946 \\

% hubei-7days & \textbf{0.959} & 0.902 & 0.912  & 0.958  \\

% hunan-7days & \textbf{0.955} & 0.935 & 0.930 & 0.953 \\

Hubei (55 days) & \textbf{0.052}  & 0.066  & 0.063 & 0.063  \\

Hunan (55 days) & 0.046 & \textbf{0.044}  & 0.054 & 0.054 \\

Hubei (7 days) & \textbf{0.041} & 0.098 & 0.088  & 0.042  \\

Hunan (7 days) & \textbf{0.045} & 0.065 & 0.070 & 0.047 \\

Bear (x days) & \textbf{0.027} & 0.056 &  \\

Eagle (x days) & \textbf{0.058} & 0.065 &  \\

Fox (x days) & \textbf{0.025} & 0.056 &  \\
\hline
% henan & \textbf{0.941} & \textbf{0.} &  0.918 & 0.  & 0.944 &  & 0.944 &   \\
% jiangxi& \textbf{0.956} & \textbf{0.} & 0.947 & 0.  & 0.921 &  & 0.922 &   \\

% ningbo & \textbf{0.932} & \textbf{0.}  & 0.882 & 0.  & 0.960 &  & 0.947 &  \\

%  yinzhou & 336 & 0.214 & 0.329 &\textbf{0.212} &\textbf{0.313} &0.231 &0.338 &0.300  &0.394  &0.280 &0.380  &0.350  & 0.433    \\
% xiangshan & 720 & 0.246 & 0.355 &\textbf{0.231} &\textbf{0.343} &0.254  &0.361  &0.373  &0.439 &0.283  &0.376  &0.340  &0.420     \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} 
% beilun &96  & 0.148 & 0.278 &\textbf{0.139} &\textbf{0.276} &0.197  &0.323  &0.847  &0.752  &0.968  &0.812  &1.065  &0.829    \\
% \bottomrule
\end{tabular}
\label{tab:benchmark_extreme}
% }
% \end{adjustwidth}
\end{footnotesize}
\end{table}
%}

==> tables/tab_dataset_public.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table}[h]
\centering
\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Summary of datasets.}
\scalebox{0.9}{
\begin{tabular}{c|c|cccc}
% \toprule
% \multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{xxxx+}&\multicolumn{2}{c|}{xxxx-}&\multicolumn{2}{c|}{LightGBM}&\multicolumn{2}{c|}{Transformer}&\multicolumn{2}{c}{N-BEATS}&\multicolumn{2}{c|}{TCN or LSTM}\\
% \midrule
% \multicolumn{2}{c|}{Metric} & 
\hline
\multicolumn{2}{c|}{Dataset}& \#Features & \#Samples & Sample rate & Population \\ %& num extreme event\\
\hline
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$huazhong$}} 
\multirow{4}{*}{HZ} 
& Hubei & 14 & 86113 & 15 min & 57.7 million\\
% \cline{2-6}
         & Hunan & 14 & 86113 & 15 min & 66.4 million \\
        %  \cline{2-6}
         & Henan & 14 & 86113 & 15 min & 99.4 million \\
        %  \cline{2-6}
         & Jiangxi & 14 & 86113& 15 min & 45.2 million \\
\hline
         
% 96 & \textbf{0.203} & \textbf{0.287} &0.204 &0.288 &0.255  &0.339  &0.365  &0.453  &0.768  &0.642  &0.658  &0.619    \\

% &96  & 0.193 & 0.308 &\textbf{0.183} &\textbf{0.297} &0.201  &0.317  &0.274  &0.368  &0.258  &0.357  &0.312  &0.402    \\
% NB & Ningbo & 14 & 15424 & 15 min & 9.5 million \\
% \hline



% \hline
% \multicolumn{2}{c|}{Dataset}& Feature & Time steps & sample rate/min & population/million \\ %& num extreme event\\
% \hline
% % \midrule
% % \multirow{4}{*}{\rotatebox{90}{$huazhong$}} 
% \multirow{4}{*}{HZ} 
% & Hubei & 14 & 86113 & 15min & 57.7 million \\
% \cline{2-6}
%          & Hunan & 14 & 86113 & 15min & 66.4 million \\
%          \cline{2-6}
%          & Henan & 14 & 86113 & 15min & 99.4 million \\
%          \cline{2-6}
%          & Jiangxi & 14 & 86113& 15min & 45.2 million \\
% \hline
         
% % 96 & \textbf{0.203} & \textbf{0.287} &0.204 &0.288 &0.255  &0.339  &0.365  &0.453  &0.768  &0.642  &0.658  &0.619    \\

% % &96  & 0.193 & 0.308 &\textbf{0.183} &\textbf{0.297} &0.201  &0.317  &0.274  &0.368  &0.258  &0.357  &0.312  &0.402    \\
% NB & Ningbo & 14 & 15424 & 15min & 9.5 million \\
% \hline
% 192 &0.201 & 0.315 & \textbf{0.195} &\textbf{0.308} &0.222  &0.334  &0.296 &0.386  &0.266 &0.368  &0.348  &0.433    \\
%  yinzhou & 336 & 0.214 & 0.329 &\textbf{0.212} &\textbf{0.313} &0.231 &0.338 &0.300  &0.394  &0.280 &0.380  &0.350  & 0.433    \\
% xiangshan & 720 & 0.246 & 0.355 &\textbf{0.231} &\textbf{0.343} &0.254  &0.361  &0.373  &0.439 &0.283  &0.376  &0.340  &0.420     \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} 
% beilun &96  & 0.148 & 0.278 &\textbf{0.139} &\textbf{0.276} &0.197  &0.323  &0.847  &0.752  &0.968  &0.812  &1.065  &0.829    \\
% \bottomrule
\end{tabular}
\label{tab:dataset}
}
% \end{adjustwidth}
\end{footnotesize}
\end{table}

% \vspace{-2.5cm}
%}

==> tables/tab_feature_engineering.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[h]
\centering
\begin{footnotesize}
%\begin{adjustwidth}
\caption{Four types of features after feature engineering}
% \scalebox{0.85}{

\resizebox{0.5\linewidth}{!}{ 
\begin{tabular}{c|c|c|c}
% \toprule
\hline
{Temporal features}&\multicolumn{1}{c|}{NWP features}&\multicolumn{1}{c|}{Load\_Rolling features}&\multicolumn{1}{c|}{Difference features}\\
% \midrule
\hline
\hline
\textbf{year} &\textbf{2\_metre\_temperature} & \textbf{load\_win\_7\_offset\_192\_median}&
\textbf{2\_metre\_temperature\_diff\_offset\_192} \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$huazhong$}} 
% huazhong & \textbf{0.963} & \textbf{0.969} & 0.952 & 0.958 & 
% 0.892 & 0.896 & 0.943 & 0.949 & 0.874 & 0.879\\

% Hubei & \textbf{0.948} & \textbf{0.955} & 0.934 & 0.942 & 0.894 & 0.901 & 0.925 & 0.933 & 0.888  & 0.886    \\

% Hunan & \textbf{0.954} & \textbf{0.961} &   0.956 & 0.953 &  0.877 & 0.882 & 0.932 & 0.939 & 0.867 & 0.879   \\

% Henan & \textbf{0.941} & \textbf{0.949} &  0.918 & 0.928 & 0.895 & 0.903 & 0.901 & 0.910 & 0.872 & 0.886      \\

% Jiangxi& \textbf{0.956} & \textbf{0.962} & 0.947 & 0.955 & 0.929 & 0.936 & 0.922 & 0.930 & 0.912 & 0.920  \\

% Ningbo & \textbf{0.932} & \textbf{0.939}  & 0.882 & 0.891 &  0.930 & 0.935 & 0.902 & 0.907 & 0.910 & 0.924   \\



 \textbf{month} & \textbf{Surface\_pressure} & \textbf{load\_win\_7\_offset\_192\_mean}&
 \textbf{Surface\_pressure\_diff\_offset\_192}\\

 \textbf{day} & \textbf{Total\_cloud\_cover} & \textbf{load\_win\_7\_offset\_192\_min}&
 \textbf{Total\_cloud\_cover\_diff\_offset\_192}\\

  \textbf{is\_workday} & \textbf{Total\_precipitation} & \textbf{load\_win\_7\_offset\_192\_max}&
  \textbf{Total\_precipitation\_diff\_offset\_192}\\
  
  \textbf{is\_holiday} & \textbf{Skin\_temperature} & \textbf{load\_win\_7\_offset\_192\_std}&
  \textbf{Skin\_temperature\_diff\_offset\_192}\\
  
  \textbf{is\_weekend} & \textbf{...} & \textbf{load\_win\_7\_offset\_192\_skew}&
  \textbf{...}\\
  
  \textbf{day\_of\_month\_sin} & \textbf{...} & \textbf{load\_win\_7\_offset\_192\_q025}&
  \textbf{...}\\
  
  \textbf{...} & \textbf{...} & \textbf{...}&
  \textbf{...}\\

\hline
%  yinzhou & 336 & 0.214 & 0.329 &\textbf{0.212} &\textbf{0.313} &0.231 &0.338 &0.300  &0.394  &0.280 &0.380  &0.350  & 0.433    \\
% xiangshan & 720 & 0.246 & 0.355 &\textbf{0.231} &\textbf{0.343} &0.254  &0.361  &0.373  &0.439 &0.283  &0.376  &0.340  &0.420     \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} 
% beilun &96  & 0.148 & 0.278 &\textbf{0.139} &\textbf{0.276} &0.197  &0.323  &0.847  &0.752  &0.968  &0.812  &1.065  &0.829    \\
% \bottomrule
\end{tabular}
}
\label{tab:feature_engineering}
% }
%\end{adjustwidth}
\end{footnotesize}
\end{table*}
%}

==> tables/tab_features_before.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[h]
\centering
\begin{footnotesize}
%\begin{adjustwidth}
\caption{Attributes}
% \scalebox{0.85}{

% \resizebox{0.2\linewidth}{!}{ 
\begin{tabular}{c|c}
% \toprule
\hline
{NWP attributes}&\multicolumn{1}{c|}{loads}\\
% \midrule
\hline
\hline
 \textbf{2\_metre\_temperature} & \textbf{hubei}  \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$huazhong$}} 
% huazhong & \textbf{0.963} & \textbf{0.969} & 0.952 & 0.958 & 
% 0.892 & 0.896 & 0.943 & 0.949 & 0.874 & 0.879\\

% Hubei & \textbf{0.948} & \textbf{0.955} & 0.934 & 0.942 & 0.894 & 0.901 & 0.925 & 0.933 & 0.888  & 0.886    \\

% Hunan & \textbf{0.954} & \textbf{0.961} &   0.956 & 0.953 &  0.877 & 0.882 & 0.932 & 0.939 & 0.867 & 0.879   \\

% Henan & \textbf{0.941} & \textbf{0.949} &  0.918 & 0.928 & 0.895 & 0.903 & 0.901 & 0.910 & 0.872 & 0.886      \\

% Jiangxi& \textbf{0.956} & \textbf{0.962} & 0.947 & 0.955 & 0.929 & 0.936 & 0.922 & 0.930 & 0.912 & 0.920  \\

% Ningbo & \textbf{0.932} & \textbf{0.939}  & 0.882 & 0.891 &  0.930 & 0.935 & 0.902 & 0.907 & 0.910 & 0.924   \\



 \textbf{Surface\_pressure} & \textbf{hunan}  \\

 \textbf{Total\_cloud\_cover} & \textbf{henan}  \\

   \textbf{Total\_precipitation} & \textbf{jiangxi}  \\
  
  \textbf{Skin\_temperature} & \textbf{ningbo}  \\
  
   
  

  
  \textbf{...} & \textbf{...}  \\

\hline
%  yinzhou & 336 & 0.214 & 0.329 &\textbf{0.212} &\textbf{0.313} &0.231 &0.338 &0.300  &0.394  &0.280 &0.380  &0.350  & 0.433    \\
% xiangshan & 720 & 0.246 & 0.355 &\textbf{0.231} &\textbf{0.343} &0.254  &0.361  &0.373  &0.439 &0.283  &0.376  &0.340  &0.420     \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} 
% beilun &96  & 0.148 & 0.278 &\textbf{0.139} &\textbf{0.276} &0.197  &0.323  &0.847  &0.752  &0.968  &0.812  &1.065  &0.829    \\
% \bottomrule
\end{tabular}


\label{tab:before_engineering}
% }
%\end{adjustwidth}
\end{footnotesize}
\end{table*}
%}
